Towards In-Context Tone Style Transfer with A Large-Scale Triplet Dataset

Tone style transfer for photo retouching aims to adapt the stylistic tone of the reference image to a given content image. However, the lack of high-quality large-scale triplet datasets with stylized ground truth forces existing methods to rely on self-supervised or proxy objectives, which limits model capability. To mitigate this gap, we design a data construction pipeline to build TST100K, a large-scale dataset of 100,000 content-reference-stylized triplets. At the core of this pipeline, we train a tone style scorer to ensure strict stylistic consistency for each triplet. In addition, existing methods typically extract content and reference features independently and then fuse them in a decoder, which may cause semantic loss and lead to inappropriate color transfer and degraded visual aesthetics. Instead, we propose ICTone, a diffusion-based framework that performs tone transfer in an in-context manner by jointly conditioning on both images, leveraging the semantic priors of generative models for semantic-aware transfer. Reward feedback learning using the tone style scorer is further incorporated to improve stylistic fidelity and visual quality. Experiments demonstrate the effectiveness of TST100K, and ICTone achieves state-of-the-art performance on both quantitative metrics and human evaluations. The project page is available online: https://dengyuhai.github.io/ICTone_Project/.

==> figures/AblationVis.tex <==
\begin{figure*}[tb]
  \centering
  \fbox{\rule{0pt}{3.in} \rule{0.97\linewidth}{0pt}}
  \caption{Visual comparison.}
  \label{fig:vis_compare}
\end{figure*}

==> figures/ModelPipeline.tex <==
% \begin{figure}[tb]
% 	\centering
% 	\includegraphics[width=1.0\linewidth]{figures/ModelPipeline.png}
% 	\caption{Overview of the in-context model training pipeline.}
% 	\label{fig:modelpipeline}
% \end{figure}
\begin{wrapfigure}[17]{r}{0.50\textwidth}
  \centering
  \vspace{-8mm}
  \includegraphics[width=\linewidth]{figures/ModelPipeline_lq.jpg}
  \caption{Overview of the in-context model training pipeline.}
  \label{fig:modelpipeline}
%   \vspace{-2.5\baselineskip}
	% \vspace{-10mm}
\end{wrapfigure}


==> figures/Motivation.tex <==
\begin{figure}[!tbp]
  \centering
  \fbox{\rule{0pt}{1.7in} \rule{.97\linewidth}{0pt}}
  \caption{Motivation}
  \label{fig:Motivation}
\end{figure}

==> figures/Pipeline.tex <==
\begin{figure*}[tb]
  \centering
  \includegraphics[width=1.0\linewidth]{figures/ModelPipeline.png}
  \caption{Overview of the UniTone training pipeline. Our framework includes (left) in-context transfer model training, which formulates color style transfer as an inpainting-based generation task, and (right) tone style discriminator training, combining weakly-supervised contrastive learning with human preference refinement for perceptual tone alignment.}
  \label{fig:pipeline}
\end{figure*}

==> figures/Visualization.tex <==
\begin{figure*}[tb]
  \centering
  \fbox{\rule{0pt}{2.6in} \rule{.97\linewidth}{0pt}}
  \caption{Visualization}
  \label{fig:Visualization}
\end{figure*}

==> figures/dataset_overview.tex <==
% \begin{wrapfigure}{r}{0.55\textwidth}
%   \centering
%   \vspace{-5mm}
%   \includegraphics[width=\linewidth]{figures/dataset_overview2.jpg}
%   \caption{The distribution of TST2K benchmark.}
%   \label{fig:dataset_overview}
% %   \vspace{-2.5\baselineskip}
%     % \vspace{-12mm}
% \end{wrapfigure}

\begin{wrapfigure}[13]{r}{0.55\textwidth}
  \centering
  \vspace{-6mm}
  \includegraphics[width=\linewidth]{figures/dataset_overview2.jpg}
  \caption{The distribution of TST2K benchmark.}
  \label{fig:dataset_overview}
\end{wrapfigure}


==> tables/Compare_CRT2K.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
	%	\small
	\centering
	\caption{Quantitative comparisons with state-of-the-art methods on the CRT-2K benchmarks. UniTone achieves the best overall performance in tone consistency, color difference, and aesthetic quality, while maintaining competitive content preservation. Methods marked with $^*$ denote retraining on our paired dataset, which further improves their performance.}
	\begin{tabular}{llllllll}
		\hline
		\multirow{2}{*}{Method}       & \multicolumn{7}{c}{PST50}                                             \\ \cline{2-8} 
		& CP \(\uparrow\)     & CP\_GT\(\uparrow\)          & TC \(\uparrow\)              & TC\_GT & \(\Delta E \downarrow\) & CD \(\downarrow\)     & Aes\(\uparrow\)       \\ \hline
		WCT$^2$~\cite{yoo2019photorealistic}        &0.6818 & 0.6482          & 0.6797 & 0.6584 & 16.34   & 5.574 & 0.2381 \\
		PhotoNAS~\cite{an2020ultrafast}             &0.6901 & 0.6757          & 0.5375 & 0.5090  & 32.87   & 8.566 & 0.2293 \\
		MKL~\cite{pitie2007linear}                  &0.7363 & 0.7305 & 0.7618          & 0.7646 & 0.7026 & 16.12   & 5.241 \\
		PhotoWCT~\cite{li2018closed}                &0.6596 & 0.6477          & 0.8156 & 0.7459 & 20.83   & 6.487 & 0.2279 \\
		DeepPreset {[}8{]}                          &0.7248 & 0.6566          & 0.5700   & 0.6197 & 16.90   & 5.679 & 0.1147 \\
		ModFlows~\cite{larchenko2025color}          &0.774  & 0.7334          & 0.6929 & 0.6689 & 15.52   & 5.651 & 0.2774 \\
		IPST~\cite{liu2023universal}                &0.7576 & 0.7275          & 0.6827 & 0.6547 & 14.08   & 5.484 & 0.2344 \\
		RLPixTuner~\cite{wu2024goal}                &\textbf{0.8081} & 0.6789          & 0.4775 & 0.5021 & 21.51   & 7.445 & 0.1946 \\
		SA-LUT~\cite{gong2025sa}                    &0.7037 & 0.7697          & 0.7407 & \underline{0.7625} & \textbf{11.25}   & \underline{4.483} & 0.2048 \\
		CAP-VSTNet~\cite{wen2023cap}                &0.7040  & 0.7384          & \underline{0.7693} & 0.7132 & 16.21   & 5.350  & 0.2705 \\
		CAP-VSTNet$^*$~\cite{wen2023cap}            &0.7801 & 0.7545          & 0.7074 & 0.7312 & 14.45   & 4.937 & \underline{0.2779} \\
		Neural Preset~\cite{ke2023neural}           &0.742  & 0.6502          & 0.6086 & 0.5716 & 19.53   & 6.965 & 0.1454 \\
		Neural Preset$^*$~\cite{ke2023neural}       &\underline{0.7919} & 0.6914          & 0.6087 & 0.6199 & 17.81   & 6.157 & 0.1714 \\
		Ours                                        &0.7323 & \textbf{0.7902} & \textbf{0.8799} & \textbf{0.8529} & \underline{12.81}   & \textbf{4.448} & \textbf{0.2820}  \\ \hline
		GT                                          &0.7209 & 1               & 0.8536 & 1      & 0       & 0     & 0.3305 \\ \hline
	\end{tabular}
\end{table*}

==> tables/Compare_PST50.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
	%	\small
%	\footnotesize
	\centering
	\caption{Quantitative comparisons with state-of-the-art methods on the PST50 benchmarks. UniTone achieves the best overall performance in tone consistency, color difference, and aesthetic quality, while maintaining competitive content preservation. Methods marked with $^*$ denote retraining on our paired dataset, which further improves their performance.}
	\begin{tabular}{llllllll}
		\hline
		\multirow{2}{*}{Method} & \multicolumn{7}{c}{TST2000}  \\ \cline{2-8} 
		& CP \(\uparrow\)     & CP\_GT\(\uparrow\)          & TC \(\uparrow\)              & TC\_GT & \(\Delta E \downarrow\) & CD \(\downarrow\)     & Aes\(\uparrow\)       \\ \hline
		WCT$^2$~\cite{yoo2019photorealistic}           & 0.4116 & 0.3952          & 0.5655          & 0.5651 & 15.13   & 4.991  & 0.7136  \\
		PhotoNAS~\cite{an2020ultrafast}                & 0.7193 & 0.6721          & 0.5429          & 0.5232 & 19.57   & 6.183  & 0.6347  \\
		MKL~\cite{pitie2007linear}                   & 0.7809 & 0.7511          & 0.6353          & 0.6143 & 12.67   & 4.694  & 0.7363 \\ 
		PhotoWCT~\cite{li2018closed}                 & 0.6126 & 0.5852          & \underline{0.7030}           & 0.6700   & 21.35   & 7.021  & 0.6788  \\
		DeepPreset {[}8{]}                           & \textbf{0.8889} & \underline{0.7728}          & 0.6118          & 0.6635 & 8.205   & 4.108  & 0.7567 \\
		ModFlows~\cite{larchenko2025color}           & 0.6949 & 0.6908          & 0.6876          & 0.6659 & 12.43   & 4.945  & 0.7500   \\
		IPST~\cite{liu2023universal}                 & 0.7749 & 0.7364          & 0.6231          & 0.6282 & 9.648   & 4.326  & 0.7081  \\
		RLPixTuner~\cite{wu2024goal}                 & 0.7324 & 0.6815          & 0.2497          & 0.2787 & 25.61   & 7.514  & 0.6354\\
		SA-LUT~\cite{gong2025sa}                     & 0.6695 & 0.7082          & 0.5254          & 0.5573 & 11.10    & 4.929  & 0.6507  \\
		CAP-VSTNet~\cite{wen2023cap}                 & 0.7148 & 0.7013          & 0.6245          & 0.6084 & 11.87   & 4.665  & 0.7175  \\
		CAP-VSTNet$^*$~\cite{wen2023cap}             & 0.8303 & 0.7665          & 0.6505          & \underline{0.6717} & 7.359   & \underline{3.663}  & 0.7721 \\
		Neural Preset~\cite{ke2023neural}            & 0.8314 & 0.748           & 0.5249          & 0.5282 & 10.51   & 4.713  & 0.7551  \\
		Neural Preset$^*$~\cite{ke2023neural}        & \underline{0.8579} & 0.7707          & 0.6058          & 0.6248 & \underline{7.886}   & 3.860   & \underline{0.7808}  \\
		Ours                                         & 0.7285 & \textbf{0.8644} & \textbf{0.8788} & \textbf{0.9280}  & \textbf{5.776}   & \textbf{2.634}  & \textbf{0.7904}   \\ \hline
		GT                                           & 0.7472 & 1               & 0.8905          & 1      & 0       & 0      & 0.7978  \\ \hline
	\end{tabular}
\end{table*}

==> tables/Compare_back.tex <==
\begin{table*}[t]
    \centering
    \caption{Quantitative comparisons with state-of-the-art methods.}
    \begin{tabular}{llllllllllll} 
    \toprule
    \multirow{2}{*}{\centering Method} & \multicolumn{5}{c}{UCST} & \multicolumn{5}{c}{PST50} \\ \cmidrule(lr){2-6} \cmidrule(lr){7-11}
                            & CP $\uparrow$ & TC $\uparrow$ & $\Delta E \downarrow$ & CD $\downarrow$ &  Ase $\uparrow$
                            & CP $\uparrow$ & TC $\uparrow$ & $\Delta E \downarrow$ & CD $\downarrow$ & Ase $\uparrow$ \\ \midrule
    WCT$^2$~\cite{yoo2019photorealistic}   &0.3886               &0.5447               &15.79                      &5.106                 &0.8123  &0.6818               &0.6797               &16.34                      &5.574                 &0.2381\\
    PhotoNAS~\cite{an2020ultrafast}        &0.7144               &0.5267               &19.04                      &6.074                 &0.7076  &0.6901               &0.5375               &32.87                      &8.566                 &0.2293 \\
    MKL~\cite{pitie2007linear}              &0.7814               &0.6180               &13.12                      &4.794                 &0.8378  &0.7305               &0.7646               &16.12                      &5.241                 &0.2742\\ %\midrule
    PhotoWCT~\cite{li2018closed}            &0.6126               &0.7030               &21.35                      & 7.021                &0.6788  &0.6596               &0.6156               &20.83                      &6.487                 &0.2279 \\
    DeepPreset~\cite{ho2021deep}            &0.1187               &0.3716               &38.88                      &9.260                 &0.8143   &0.7248               &0.5700               &16.90                      &5.679                 &0.1147\\ %\midrule
    ModFlows~\cite{larchenko2025color}       &0.6910               &0.6810               &12.86                      &5.048                 &0.8432   &0.7740               &0.6929               &15.52                      &5.651                 &0.2774\\ %\midrule
    IPST~\cite{liu2023universal}             &0.7770               &0.6143               &9.692                      &4.336                 &0.8079    &0.7576               &0.6827               &14.08                      &5.484                 &0.2344\\
    RLPixTuner~\cite{wu2024goal}             &0.7225               &0.2358               &26.47                      &7.668                 &0.7160    &0.8081               &0.4775               &21.51                      &7.445                 &0.1946\\ %\midrule
    SA-LUT~\cite{gong2025sa}               &0.6566               &0.5110               &10.69                      &4.859                 &0.7316 &0.7037               &0.7407               &11.25                      &4.86                 &0.2048\\
    CAP-VSTNet~\cite{wen2023cap}           &0.7145               &0.6083               &12.21                      &4.749                 &0.8186   &0.7040               &0.7693               &16.21                      &5.350                 &0.2705\\
    CAP-VSTNet$^*$~\cite{wen2023cap}      &0.7801               &0.7074               &14.45                      &4.937                 &0.2819   &0.8357               &0.6359               &7.161                      &3.646                 &0.8785 \\
    Neural Preset~\cite{ke2023neural}     &0.7420               &0.6086               &19.53                      &6.965                 &0.1454   &0.8265               &0.5638               & 10.34                     &4.512                 &0.8631 \\
    Neural Preset$^*$~\cite{ke2023neural}        &0.8567               &0.6087               &7.609                      &3.785                 &0.8711  &0.7919               &0.4575      &17.81         &6.157                      & 0.1714\\
    Ours               &0.7014               &0.8773               &5.553                      &2.854                 &0.8789  &0.7348               &0.8245               &12.34                     &4.416                 &0.3283\\ \midrule
    GT               &0.7379               &0.8888               &0.000                      &0.000  &0.8986  &0.7209               &0.8536               &0.000                     &0.000                 &0.3305\\
    \bottomrule
    \end{tabular}
    \label{tab:comp_meadravdess}
\end{table*}

==> tables/Notations.tex <==
\begin{table}[h]
    \centering
    \caption{\textbf{Main notations} in the manuscripts with the corresponding descriptions.}
    \begin{tabular}{cl}
    \toprule
    Notation & Discription \\
    \midrule
    \midrule
    $a_i$ & test notation 1 \\
    $b_j$ & test notation 2 \\
    $c_k$ & test notation 3 \\
    \bottomrule
    \end{tabular}
    \label{tab:notations}
\end{table}
